Conversational Agents to Facilitate Deliberation on Harmful Content in WhatsApp Groups

WhatsApp groups have become a hotbed for the propagation of harmful content including misinformation, hate speech, polarizing content, and rumors, especially in Global South countries. Given the platform's end-to-end encryption, moderation responsibilities lie on group admins and members, who rarely contest such content. Another approach is fact-checking, which is unscalable, and can only contest factual content (e.g., misinformation) but not subjective content (e.g., hate speech). Drawing on recent literature, we explore deliberation -- open and inclusive discussion -- as an alternative. We investigate the role of a conversational agent in facilitating deliberation on harmful content in WhatsApp groups. We conducted semi-structured interviews with 21 Indian WhatsApp users, employing a design probe to showcase an example agent. Participants expressed the need for anonymity and recommended AI assistance to reduce the effort required in deliberation. They appreciated the agent's neutrality but pointed out the futility of deliberation in echo chamber groups. Our findings highlight design tensions for such an agent, including privacy versus group dynamics and freedom of speech in private spaces. We discuss the efficacy of deliberation using deliberative theory as a lens, compare deliberation with moderation and fact-checking, and provide design recommendations for future such systems. Ultimately, this work advances CSCW by offering insights into designing deliberative systems for combating harmful content in private group chats on social media.

==> tables/design_findings_summary.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Design Dimension}} & \multicolumn{1}{c|}{\textbf{Key Findings}} \\ \hline
\multirow{2}{*}{Activation} & \begin{tabular}[c]{@{}l@{}}Freedom of speech in private spaces vs calling out hate speech\\ (e.g., homophobic content)\end{tabular} \\ \cline{2-2} 
 & Trade-off between privacy and group dynamics \\ \hline
\multirow{3}{*}{Participation} & Even participation vs including minority opinions \\ \cline{2-2} 
 & Combating harmful content while minimising workload on users \\ \cline{2-2} 
 & Platform-level crowdsourcing not suitable for context-specific private spaces \\ \hline
\multirow{2}{*}{Duration} & Access (giving time to discuss) vs context (conversation may move on) \\ \cline{2-2} 
 & Duration may unexpectedly creep in bias into the deliberation system \\ \hline
\end{tabular}
\caption{Summary of key findings about the design of the agent}
\label{tab:design-key-findings}
\vspace{-0.5cm}
\end{table}
